From Human Judgements to Predictive Models: Unravelling Acceptability in Code-Mixed Sentences

Current computational approaches for analysing or generating code-mixed sentences do not explicitly model ``naturalness'' or ``acceptability'' of code-mixed sentences, but rely on training corpora to reflect distribution of acceptable code-mixed sentences. Modelling human judgement for the acceptability of code-mixed text can help in distinguishing natural code-mixed text and enable quality-controlled generation of code-mixed text. To this end, we construct Cline - a dataset containing human acceptability judgements for English-Hindi~(en-hi) code-mixed text. Cline is the largest of its kind with 16,642 sentences, consisting of samples sourced from two sources: synthetically generated code-mixed text and samples collected from online social media. Our analysis establishes that popular code-mixing metrics such as CMI, Number of Switch Points, Burstines, which are used to filter/curate/compare code-mixed corpora have low correlation with human acceptability judgements, underlining the necessity of our dataset. Experiments using Cline demonstrate that simple Multilayer Perceptron (MLP) models when trained solely using code-mixing metrics as features are outperformed by fine-tuned pre-trained Multilingual Large Language Models (MLLMs). Specifically, among Encoder models XLM-Roberta and Bernice outperform IndicBERT across different configurations. Among Encoder-Decoder models, mBART performs better than mT5, however Encoder-Decoder models are not able to outperform Encoder-only models. Decoder-only models perform the best when compared to all other MLLMS, with Llama 3.2 - 3B models outperforming similarly sized Qwen, Phi models. Comparison with zero and fewshot capabilitites of ChatGPT show that MLLMs fine-tuned on larger data outperform ChatGPT, providing scope for improvement in code-mixed tasks. Zero-shot transfer from En-Hi to En-Te acceptability judgments are better than random baselines.

==> tables/01-dataset-stats.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{booktabs}

% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{booktabs}

% \usepackage{graphicx}

\begin{table}[b]
\caption{Dataset Statistics. On average, annotators took $\approx 3$x more time to annotate an OSN sample when compared to a GCM sample.}
\resizebox{0.6\linewidth}{!}{%
\begin{tabular}{ccc} 
\hline
\multicolumn{1}{l}{}                                                       & \begin{tabular}[c]{@{}c@{}}\textbf{Number of }\\\textbf{Samples}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Mean Annotation }\\\textbf{Time per sample}\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Synthetic Code Mix Text \\(GCM)\end{tabular}    & 10,726                                                                        & 29.51 seconds                                                                                \\ 
\hline
\begin{tabular}[c]{@{}c@{}}Online Social Network Text \\(OSN)\end{tabular} & 5,916                                                                         & 91.20 seconds                                                                                \\
\hline
\end{tabular}
}
\label{tab:dataset-stats}

\end{table}
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccc} 
% \hline
% \multicolumn{1}{l}{}    & \begin{tabular}[c]{@{}c@{}}\textbf{Number of }\\\textbf{Samples}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Mean Annotation }\\\textbf{Time per sample}\end{tabular}  \\ 
% \hline
% Synthetic Code Mix Text (GCM)      & 10,726                                                                         & 29.51 seconds                                                                                \\ 
% \hline
% Online Social Network Text (OSN) & 5,916                                                                          & 91.20 seconds                                                                                \\
% \hline
% \end{tabular}
% }
% \caption{Dataset Statistics. On average, annotators took $\approx 3$x more time to annotate an OSN sample when compared to a GCM sample.}
% \label{tab:dataset-stats}

% \end{table}

% % \usepackage{tabularray}
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tblr}{
%   row{even} = {c},
%   row{3} = {c},
%   cell{1}{1} = {c},
%   cell{1}{3} = {c},
%   cell{1}{4} = {c},
%   cell{2}{1} = {r=2}{},
%   cell{5}{2} = {c},
%   hline{1,6} = {-}{0.08em},
%   hline{2,4-5} = {-}{0.05em},
%   hline{3} = {2-4}{0.03em},
% }
% {\textbf{Acceptability }\\\textbf{Judgements }} &                         & {\textbf{Number of }\\\textbf{Samples}} & {\textbf{Mean Annotation }\\\textbf{Time (Std. Dev)}} \\
% \textbf{5-point Rating Scale}                                 & Social Network Text     & 11753                                   & 29.51 seconds                                         \\
%                                                 & Synthetic Code Mix Text & 5101                                    & 91.20 seconds                                         \\
% \textbf{Binary}                               & Synthetic Code Mix Text & 3684                                    & ~-                                                    \\
%                                                 & \textbf{Total}          &                                         &                                                       
% \end{tblr}
% }
% \caption{Dataset Statistics}
% \label{tab:dataset-stats}
% \end{table}


%GCM2
% 2596 (tanish+) + 750 (team 3-6) + 338 (divij)
% GCM1
% In [6]: traindf.shape, validdf.shape, testdf.shape
% Out[6]: ((8226, 86), (1176, 86), (2351, 86))

% OSN
% In [5]: traindf.shape, validdf.shape, testdf.shape
% Out[5]: ((3570, 48), (510, 48), (1021, 48))

% \begin{table}\label{tab:dataset-stats}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{ccll} 
% \toprule
% \begin{tabular}[c]{@{}c@{}}\textbf{Acceptability }\\\textbf{Judgements }\end{tabular} & \multicolumn{1}{l}{}    & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Number of }\\\textbf{Samples}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Mean Annotation }\\\textbf{Time (Std. Dev)}\end{tabular}}  \\ 
% \midrule
% \multirow{2}{*}{\textbf{Rating}}                                                      & Social Network Text     &                                                                                                   &                                                                                                                  \\ 
% \cmidrule{2-4}
%                                                                                       & Synthetic Code Mix Text &                                                                                                   &                                                                                                                  \\ 
% \midrule
% \textbf{Choosing}                                                                     & Synthetic Code Mix Text &                                                                                                   &                                                                                                                  \\ 
% \midrule
% \multicolumn{1}{l}{}                                                                  & \textbf{Total}          &                                                                                                   &                                                                                                                  \\
% \bottomrule
% \end{tabular}
% }
% \caption{Dataset Statistics}

% \end{table}





% \begin{table*}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cclll} 
% \toprule
% \begin{tabular}[c]{@{}c@{}}\textbf{Acceptability }\\\textbf{Judgements }\end{tabular} & \multicolumn{1}{l}{}    & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Number of }\\\textbf{Samples}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Number of }\\\textbf{Annotations}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{Mean Annotation }\\\textbf{Time (Std. Dev)}\end{tabular}}  \\ 
% \midrule
% \multirow{2}{*}{\textbf{Rating}}                                                      & Social Network Text     &                                                                                                   &                                                                                                       &                                                                                                                  \\ 
% \cmidrule{2-5}
%                                                                                       & Synthetic Code Mix Text &                                                                                                   &                                                                                                       &                                                                                                                  \\ 
% \midrule
% \textbf{Choosing}                                                                     & Synthetic Code Mix Text &                                                                                                   &                                                                                                       &                                                                                                                  \\ 
% \midrule
% \multicolumn{1}{l}{}                                                                  & \textbf{Total}          &                                                                                                   &                                                                                                       &                                                                                                                  \\
% \bottomrule
% \end{tabular}
% }
% \caption{Dataset Statistics}

% \end{table*}

% % \usepackage{graphicx}


% \begin{table}
% \centering
% \caption{Dataset Statistics}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{llll}
% \multicolumn{4}{c}{\textbf{Acceptability Judgements - Score}}                                                                                                 \\ 
% \hline
%                                    & \multicolumn{1}{c}{\textbf{\# Samples}} & \multicolumn{1}{c}{\textbf{\# Annotations}} & Mean Annotation Time (Std. Dev)  \\ 
% \hline
% Social Network Text                &                                         &                                             &                                  \\
% Synthetic Code Mix Text            &                                         &                                             &                                  \\ 
% \hline
% \multicolumn{4}{c}{\textbf{Acceptability Judgements - Rate}}                                                                                                  \\ 
% \hline
% \multicolumn{4}{l}{Synthetic Code Mix Text}                                                                                                                   \\ 
% \hline
% \multicolumn{1}{c}{\textbf{Total}} &                                         &                                             &                                  \\
% \hline
% \end{tabular}
% }
% \end{table}

% % \begin{table}
% % \centering
% % \resizebox{0.5\textwidth}{!}{
% % \begin{tabular}{lll}
% % \multicolumn{3}{c}{\textbf{Acceptability Judgements - Score}}                                                               \\ 
% % \hline
% %                                    & \multicolumn{1}{c}{\textbf{\# Samples}} & \multicolumn{1}{c}{\textbf{\# Annotations}}  \\ 
% % \hline
% % Social Network Text                &                                         &                                              \\
% % Synthetic Code Mix Text            &                                         &                                              \\ 
% % \hline
% % \multicolumn{3}{c}{\textbf{Acceptability Judgements - Rate}}                                                                \\ 
% % \hline
% % \multicolumn{3}{l}{Synthetic Code Mix Text}                                                                                 \\ 
% % \hline
% % \multicolumn{1}{c}{\textbf{Total}} &                                         &                                              \\
% % \hline
% % \end{tabular}
% % }
% % \caption{Dataset Statistics}

% % \end{table}

==> tables/03-results.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage{tabularray}

% \usepackage{tabularray}
\begin{table}[!h]
\caption{Performance measure for GCM and OSN data, using different baselines and models. Fine-tuned MLLMs outperform human baselines, and regression models trained on only code-mix metrics. $\downarrow$ indicates lower number shows better performance.}
\label{tab:results_seperate_training_withChatGPT}
\centering
\resizebox{0.75\linewidth}{!}{%
\begin{tblr}{
  row{14} = {c},
  row{16} = {c},
  cell{1}{3} = {c=2}{c},
  cell{1}{5} = {c=2}{c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{7}{1} = {r=2}{},
  cell{7}{3} = {c},
  cell{7}{4} = {c},
  cell{7}{5} = {c},
  cell{7}{6} = {c},
  cell{8}{3} = {c},
  cell{8}{4} = {c},
  cell{8}{5} = {c},
  cell{8}{6} = {c},
  cell{9}{1} = {r=2}{},
  cell{9}{3} = {c},
  cell{9}{4} = {c},
  cell{9}{5} = {c},
  cell{9}{6} = {c},
  cell{10}{3} = {c},
  cell{10}{4} = {c},
  cell{10}{5} = {c},
  cell{10}{6} = {c},
  cell{11}{1} = {r=2}{},
  cell{11}{3} = {c},
  cell{11}{4} = {c},
  cell{11}{5} = {c},
  cell{11}{6} = {c},
  cell{12}{3} = {c},
  cell{12}{4} = {c},
  cell{12}{5} = {c},
  cell{12}{6} = {c},
  cell{13}{1} = {r=2}{},
  cell{13}{2} = {c},
  cell{13}{3} = {c},
  cell{13}{4} = {c},
  cell{13}{5} = {c},
  cell{13}{6} = {c},
  cell{15}{1} = {r=2}{},
  cell{15}{2} = {c},
  cell{15}{3} = {c},
  cell{15}{4} = {c},
  cell{15}{5} = {c},
  cell{15}{6} = {c},
  hline{1-3,5,7,13,17} = {-}{},
}
                                                &            & GCM               &                  & OSN               &                  \\
                                                &            & RMSE $\downarrow$ & MAE $\downarrow$ & RMSE $\downarrow$ & MAE $\downarrow$ \\
Random Predictions                              &            & 1.54              & 1.25             & 1.78              & 1.47             \\
Human Annotations Baseline                      &            & 1.05              & 0.78             & 0.95              & 0.78             \\
{Feed Forward Network\\Using~ Code-Mix Metrics} &            & 0.97              & 0.83             & 1.42              & 1.01             \\
~~~~~~~~~~ + MLLM Perplexity Scores             &            & 0.97              & 0.84             & 1.52              & 1.04             \\
XLM-Roberta                                     & Romanised  & 0.8               & 0.62             & 1.08              & 0.78             \\
                                                & Normalised & 0.74              & 0.58             & \textbf{1.01}     & \textbf{0.743}   \\
BERNICE                                         & Romanised  & 0.79              & 0.62             & 1.02              & 0.77             \\
                                                & Normalised & \textbf{0.72}     & \textbf{0.57}    & 1.05              & 0.78             \\
IndicBERT                                       & Romanised  & 0.88              & 0.7              & 1.17              & 0.94             \\
                                                & Normalised & 0.87              & 0.69             & 1.2               & 0.97             \\
ChatGPT-3.5 - ZeroShot                          & Romanised  & 1.20              & 0.95             & 1.28              & 1.02             \\
                                                & Normalised & 1.22              & 0.96             & 1.39              & 1.12             \\
ChatGPT-3.5 - 5-Shot                            & Romanised  & 1.16              & 0.94             & 1.75              & 1.48             \\
                                                & Normalised & 1.09              & 0.87             & 1.71              & 1.46             
\end{tblr}
}

\end{table}

% \usepackage{tabularray}
% \begin{table}
% \centering
% \resizebox{0.5\linewidth}{!}{%
% \begin{tblr}{
%   row{14} = {c},
%   row{16} = {c},
%   cell{1}{3} = {c=2}{c},
%   cell{1}{5} = {c=2}{c},
%   cell{3}{3} = {r},
%   cell{3}{4} = {r},
%   cell{3}{5} = {r},
%   cell{3}{6} = {r},
%   cell{4}{3} = {r},
%   cell{4}{4} = {r},
%   cell{4}{5} = {r},
%   cell{4}{6} = {r},
%   cell{5}{3} = {r},
%   cell{5}{4} = {r},
%   cell{5}{5} = {r},
%   cell{5}{6} = {r},
%   cell{6}{3} = {r},
%   cell{6}{4} = {r},
%   cell{6}{5} = {r},
%   cell{6}{6} = {r},
%   cell{7}{1} = {r=2}{},
%   cell{7}{3} = {r},
%   cell{7}{4} = {r},
%   cell{7}{5} = {r},
%   cell{7}{6} = {r},
%   cell{8}{3} = {r},
%   cell{8}{4} = {r},
%   cell{8}{5} = {r},
%   cell{8}{6} = {r},
%   cell{9}{1} = {r=2}{},
%   cell{9}{3} = {r},
%   cell{9}{4} = {r},
%   cell{9}{5} = {r},
%   cell{9}{6} = {r},
%   cell{10}{3} = {r},
%   cell{10}{4} = {r},
%   cell{10}{5} = {r},
%   cell{10}{6} = {r},
%   cell{11}{1} = {r=2}{},
%   cell{11}{3} = {r},
%   cell{11}{4} = {r},
%   cell{11}{5} = {r},
%   cell{11}{6} = {r},
%   cell{12}{3} = {r},
%   cell{12}{4} = {r},
%   cell{12}{5} = {r},
%   cell{12}{6} = {r},
%   cell{13}{1} = {r=2}{},
%   cell{13}{2} = {c},
%   cell{13}{3} = {c},
%   cell{13}{4} = {c},
%   cell{13}{5} = {c},
%   cell{13}{6} = {c},
%   cell{15}{1} = {r=2}{},
%   cell{15}{2} = {c},
%   cell{15}{3} = {c},
%   cell{15}{4} = {c},
%   cell{15}{5} = {c},
%   cell{15}{6} = {c},
%   hline{1-3,5,7,13,17} = {-}{},
% }
%                                                  &            & GCM  &      & OSN  &       \\
%                                                  &            & RMSE $\downarrow$ & MAE $\downarrow$ & RMSE $\downarrow$ & MAE $\downarrow$  \\
% Random Predictions                               &            & 1.54 & 1.25 & 1.78 & 1.47  \\
% Human Annotations Baseline                       &            & 1.05 & 0.78 & 0.95 & 0.78  \\
% {Feed Forward Network\\
% Using~ Code-Mix Metrics} &            & 0.97 & 0.83 & 1.42 & 1.01  \\
% ~~~~~~~~~~ + MLLM Perplexity Scores              &            & 0.97 & 0.84 & 1.52 & 1.04  \\
% XLM-Roberta                                      & Romanised  & 0.8  & 0.62 & 1.08 & 0.78  \\
%                                                  & Normalised & 0.74 & 0.58 & \textbf{1.01} & \textbf{0.743} \\
% BERNICE                                          & Romanised  & 0.79 & 0.62 & 1.02 & 0.77  \\
%                                                  & Normalised & \textbf{0.72} & \textbf{0.57} & 1.05 & 0.78  \\
% IndicBERT                                        & Romanised  & 0.88 & 0.7  & 1.17 & 0.94  \\
%                                                  & Normalised & 0.87 & 0.69 & 1.2  & 0.97  \\
% ChatGPT-3.5 - ZeroShot                               & Romanised  & 1.20 & 0.95 & 1.28 & 1.02  \\
%                                                  & Normalised & 1.22 & 0.96 & 1.39 & 1.12  \\
% ChatGPT-3.5 - 5-Shot                                & Romanised  & 1.16 & 0.94 & 1.75 & 1.48  \\
%                                                  & Normalised & 1.09 & 0.87 & 1.71 & 1.46  
% \end{tblr}
% }
% \caption{Performance measure for GCM and OSN data, using different baselines and models. Fine-tuned MLLMs outperform human baselines, and regression models trained on only code-mix metrics. $\downarrow$ indicates lower number shows better performance.}
% \label{tab:results_seperate_training}
% \end{table}


% \begin{table}
% \centering
% \resizebox{0.5\linewidth}{!}{%
% \begin{tblr}{
%   cell{1}{3} = {c=2}{c},
%   cell{1}{5} = {c=2}{c},
%   cell{3}{3} = {r},
%   cell{3}{4} = {r},
%   cell{3}{5} = {r},
%   cell{3}{6} = {r},
%   cell{4}{3} = {r},
%   cell{4}{4} = {r},
%   cell{4}{5} = {r},
%   cell{4}{6} = {r},
%   cell{5}{3} = {r},
%   cell{5}{4} = {r},
%   cell{5}{5} = {r},
%   cell{5}{6} = {r},
%   cell{6}{3} = {r},
%   cell{6}{4} = {r},
%   cell{6}{5} = {r},
%   cell{6}{6} = {r},
%   cell{7}{1} = {r=2}{},
%   cell{7}{3} = {r},
%   cell{7}{4} = {r},
%   cell{7}{5} = {r},
%   cell{7}{6} = {r},
%   cell{8}{3} = {r},
%   cell{8}{4} = {r},
%   cell{8}{5} = {r},
%   cell{8}{6} = {r},
%   cell{9}{1} = {r=2}{},
%   cell{9}{3} = {r},
%   cell{9}{4} = {r},
%   cell{9}{5} = {r},
%   cell{9}{6} = {r},
%   cell{10}{3} = {r},
%   cell{10}{4} = {r},
%   cell{10}{5} = {r},
%   cell{10}{6} = {r},
%   cell{11}{1} = {r=2}{},
%   cell{11}{3} = {r},
%   cell{11}{4} = {r},
%   cell{11}{5} = {r},
%   cell{11}{6} = {r},
%   cell{12}{3} = {r},
%   cell{12}{4} = {r},
%   cell{12}{5} = {r},
%   cell{12}{6} = {r},
%   hline{1-3,5,7,9,11,13} = {-}{},
% }
%                                                 &            & GCM           &               & OSN           &                \\
%                                                 &            & RMSE          & MAE           & RMSE          & MAE            \\
% Random Predictions                              &            & 1.54          & 1.25          & 1.78          & 1.47           \\
% Human Annotations Baseline                      &            & 1.05          & 0.78          & 0.95          & 0.78           \\
% {Feed Forward Network\\Using~ Code-Mix Metrics} &            & 0.97          & 0.83          & 1.42          & 1.01           \\
% ~~~~~~~~~~ + MLLM Perplexity Scores             &            & 0.97          & 0.84          & 1.52          & 1.04           \\
% XLM-Roberta                                     & roman      & 0.8           & 0.62          & 1.08          & 0.78           \\
%                                                 & normalized & \textbf{0.74} & 0.58          & \textbf{1.01} & \textbf{0.743} \\
% BERNICE                                         & roman      & 0.79          & 0.62          & 1.02          & 0.77           \\
%                                                 & normalized & 0.72          & \textbf{0.57} & 1.05          & 0.78           \\
% IndicBERT                                       & roman      & 0.88          & 0.7           & 1.17          & 0.94           \\
%                                                 & normalized & 0.87          & 0.69          & 1.2           & 0.97           
% \end{tblr}
% }
% \caption{Performance measure for GCM and OSN data, using different models baselines. Fine-tuned MLLMs outperform human baselines, and regression models trained on only code-mix metrics.}
% \label{tab:results_seperate_training}
% \end{table}


% \usepackage{tabularray}
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tblr}{
%   cell{1}{3} = {c=2}{c},
%   cell{1}{5} = {c=2}{c},
%   cell{3}{3} = {r},
%   cell{3}{4} = {r},
%   cell{3}{5} = {r},
%   cell{3}{6} = {r},
%   cell{4}{3} = {r},
%   cell{4}{4} = {r},
%   cell{4}{5} = {r},
%   cell{4}{6} = {r},
%   cell{5}{3} = {r},
%   cell{5}{4} = {r},
%   cell{5}{5} = {r},
%   cell{5}{6} = {r},
%   cell{6}{3} = {r},
%   cell{6}{4} = {r},
%   cell{6}{5} = {r},
%   cell{6}{6} = {r},
%   cell{7}{1} = {r=2}{},
%   cell{7}{3} = {r},
%   cell{7}{4} = {r},
%   cell{7}{5} = {r},
%   cell{7}{6} = {r},
%   cell{8}{3} = {r},
%   cell{8}{4} = {r},
%   cell{8}{5} = {r},
%   cell{8}{6} = {r},
%   cell{9}{1} = {r=2}{},
%   cell{9}{3} = {r},
%   cell{9}{4} = {r},
%   cell{9}{5} = {r},
%   cell{9}{6} = {r},
%   cell{10}{3} = {r},
%   cell{10}{4} = {r},
%   cell{10}{5} = {r},
%   cell{10}{6} = {r},
%   cell{11}{1} = {r=2}{},
%   cell{11}{3} = {r},
%   cell{11}{4} = {r},
%   cell{11}{5} = {r},
%   cell{11}{6} = {r},
%   cell{12}{3} = {r},
%   cell{12}{4} = {r},
%   cell{12}{5} = {r},
%   cell{12}{6} = {r},
%   hline{1-3,5,7,13} = {-}{},
% }
%                                                  &            & GCM  &      & OSN  &       \\
%                                                  &            & RMSE & MAE  & RMSE & MAE   \\
% Random Predictions                               &            & 1.54 & 1.25 & 1.78 & 1.47  \\
% Human Annotations Baseline                       &            & 1.05 & 0.78 & 0.95 & 0.78  \\
% {Feed Forward Network\\
% Using~ Code-Mix Metrics} &            & 0.97 & 0.83 & 1.42 & 1.01  \\
% ~~~~~~~~~~ + MLLM Perplexity Scores              &            & 0.97 & 0.84 & 1.52 & 1.04  \\
% XLM-Roberta                                      & roman      & 0.8  & 0.62 & 1.08 & 0.78  \\
%                                                  & normalised & \textbf{0.74} & 0.58 & \textbf{1.01} & \textbf{0.743} \\
% BERNICE                                          & roman      & 0.79 & 0.62 & 1.02 & 0.77  \\
%                                                  & normalised & 0.72 & \textbf{0.57} & 1.05 & 0.78  \\
% IndicBERT                                        & roman      & 0.88 & 0.7  & 1.17 & 0.94  \\
%                                                  & normalised & 0.87 & 0.69 & 1.2  & 0.97  
% \end{tblr}
% }
% \caption{Performance measure for GCM and OSN data, using different models baselines. Fine-tuned MLLMs outperform human baselines, and regression models trained on only code-mix metrics.}
% \label{tab:results_seperate_training}

% \end{table}


% \begin{table*}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccccccccc} 
% \hline\hline
%                                                                                &                             &          & \multicolumn{4}{c}{Average Rating}                                                     & \multicolumn{4}{c}{Sum of Pair Wise Abs Diff}                                           \\ 
% \cmidrule{4-11}
%                                                                                &                             &          & \multicolumn{2}{c}{\multirow{2}{*}{OSN}} & \multicolumn{2}{c}{\multirow{2}{*}{GCM}}    & \multicolumn{2}{c}{\multirow{2}{*}{OSN}} & \multicolumn{2}{c}{\multirow{2}{*}{GCM}}     \\
%                                                                                &                             &          & \multicolumn{2}{c}{}                     & \multicolumn{2}{c}{}                        & \multicolumn{2}{c}{}                     & \multicolumn{2}{c}{}                         \\ 
% \cmidrule{4-11}
%                                                                                &                             &          & RMSE & MAE                               & RMSE                 & MAE                  & RMSE & MAE                               & RMSE                 & MAE                   \\ 
% \hline\hline
% Human Annotations Baseline                                                     &                             &          & \multicolumn{2}{c}{}                     &                      &                      & \multicolumn{2}{c}{}                     &                      &                       \\ 
% \hline\hline
% \begin{tabular}[c]{@{}l@{}}Feed-Forward Network \\- Code-mix Metrics\end{tabular} &                             &          &      &                                   &                      &                      & \multicolumn{2}{c}{}                     &                      &                       \\
% ~~~ + MLLM Perplexity scores                                                   &                             &          &      &                                   &                      &                      & \multicolumn{2}{c}{}                     &                      &                       \\ 
% \hline\hline
% \multirow{4}{*}{XLM-Roberta}                                                   & \multirow{2}{*}{roman}      & Frozen   & 1    & 0.85                              & 0.91 \textbar{} 0.91 & 0.76 \textbar{} 0.76 & 1.98 & 1.34                              & 1.84 \textbar{} 1.84 & 1.56 \textbar{} 1.56  \\
%                                                                                &                             & Unfrozen & 0.89 & 0.69                              & 0.85 \textbar{} 0.81 & 0.65 \textbar{} 0.63 & 1.92 & 1.46                              & 1.90 \textbar{} 1.89 & 1.53 \textbar{} 1.50  \\
%                                                                                & \multirow{2}{*}{normalised} & Frozen   & 1    & 0.85                              & 0.91                 & 0.76                 & 1.98 & 1.34                              & 1.84                 & 1.56                  \\
%                                                                                &                             & Unfrozen & 0.87 & 0.66                              & 0.73                 & 0.56                 & 1.9  & 1.4                               & 1.85                 & 1.56                  \\ 
% \cline{1-1}\cmidrule{2-11}
% \multirow{4}{*}{IndicBERT}                                                     & \multirow{2}{*}{roman}      & Frozen   & 3.4  & 3.3                               & 1.94 \textbar{} 1.9  & 1.74 \textbar{} 1.7  & 2.8  & 2.1                               & 2.2 \textbar{}~ 2.21 & 1.69 \textbar{} 1.73  \\
%                                                                                &                             & Unfrozen & 1    & 0.83                              & 0.88 \textbar{} 0.85 & 0.71 \textbar{} 0.69 & 1.97 & 1.46                              & 1.89 \textbar{} 1.86 & 1.53 \textbar{} 1.53  \\
%                                                                                & \multirow{2}{*}{normalised} & Frozen   & 3.3  & 3.3                               & 1.9                  & 1.69                 & 2.8  & 2.2                               & 2.2                  & 1.72                  \\
%                                                                                &                             & Unfrozen & 1.02 & 0.84                              & 0.9                  & 0.7                  & 1.96 & 1.47                              & 1.89                 & 1.53                  \\ 
% \cline{1-1}\cmidrule{2-11}
% \multirow{4}{*}{BERNICE}                                                       & \multirow{2}{*}{roman}      & Frozen   & 0.97 & 0.77                              & 0.87 \textbar{} 0.87 & 0.71 \textbar{} 0.71 & 1.92 & 1.55                              & 1.84 \textbar{} 1.84 & 1.56 \textbar{} 1.56  \\
%                                                                                &                             & Unfrozen & 0.91 & 0.73                              & 0.82 \textbar{} 0.78 & 0.63 \textbar{} 0.60 & 1.87 & 1.43                              & 1.84 \textbar{} 1.84 & 1.56 \textbar{} 1.56  \\
%                                                                                & \multirow{2}{*}{normalised} & Frozen   & 0.98 & 0.79                              & 0.87                 & 0.69                 & 1.93 & 1.57                              & 1.84                 & 1.56                  \\
%                                                                                &                             & Unfrozen & 0.91 & 0.72                              & 0.75                 & 0.57                 & 1.9  & 1.47                              & 1.84                 & 1.56                  \\
% \hline\hline
% \end{tabular}
% }
% \caption{Results: XLit | IndicTrans}
% \label{tab:results_seperate_training}
% \end{table*}
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{clllll} 
% \hline\hline
% \multicolumn{1}{l}{}                                                                   & \multicolumn{1}{c}{\textbf{OSN}} & \multicolumn{1}{c}{\textbf{GCM}} & \multicolumn{1}{c}{\textbf{OSN - GCM}} & \multicolumn{1}{c}{\textbf{GCM- OSN}} & \multicolumn{1}{c}{\textbf{GCM + OSN}}  \\ 
% \cmidrule{2-6}
% \multicolumn{1}{l}{}                                                                   & \multicolumn{5}{c}{\textbf{MSE}}                                                                                                                                                               \\ 
% \cmidrule{2-6}
% \begin{tabular}[c]{@{}c@{}}\textbf{Human Annotations }\\\textbf{Baseline}\end{tabular} &                                  &                                  &                                        &                                       &                                         \\ 
% \hline
% \textbf{Linear Regression}                                                             &                                  &                                  &                                        &                                       &                                         \\ 
% \midrule
% \textbf{XLM-R}                                                                         &                                  &                                  &                                        &                                       &                                         \\ 
% \midrule
% \textbf{IndicBERT}                                                                     &                                  &                                  &                                        &                                       &                                         \\ 
% \midrule
% \multicolumn{1}{l}{}                                                                   & \multicolumn{5}{c}{\textbf{Binary Classification}}                                                                                                                                             \\ 
% \hline
% \textbf{Linear Regression}                                                             &                                  &                                  &                                        &                                       &                                         \\ 
% \hline
% \textbf{XLM-R}                                                                         & \multicolumn{5}{l}{}                                                                                                                                                                           \\ 
% \hline
% \textbf{IndicBERT}                                                                     &                                  &                                  &                                        &                                       &                                         \\
% \hline\hline
% \end{tabular}
% }
% \caption{Results}

% \end{table}

% % % \usepackage{graphicx}
% % % \usepackage{multirow}
% % % \usepackage{booktabs}


% % \begin{table}
% % \centering
% % \caption{Dataset Statistics}
% % \resizebox{\linewidth}{!}{%
% % \begin{tabular}{cllllll} 
% % \hline\hline
% % \multicolumn{1}{l}{}                        &                       & \multicolumn{1}{c}{\textbf{OSN}} & \multicolumn{1}{c}{\textbf{GCM}} & \multicolumn{1}{c}{\textbf{OSN -\textgreater{} GCM}} & \multicolumn{1}{c}{\textbf{GCM-\textgreater{} OSN}} & \multicolumn{1}{c}{\textbf{GCM + OSN}}  \\ 
% % \midrule
% % \multirow{2}{*}{\textbf{Linear Regression}} & MSE                   &                                  &                                  &                                                      &                                                     &                                         \\ 
% % \cmidrule{2-7}
% %                                             & Binary Classification &                                  &                                  &                                                      &                                                     &                                         \\ 
% % \midrule
% % \multirow{2}{*}{\textbf{SVM Regression}}    & MSE                   &                                  &                                  &                                                      &                                                     &                                         \\ 
% % \cmidrule{2-7}
% %                                             & Binary Classification &                                  &                                  &                                                      &                                                     &                                         \\ 
% % \midrule
% % \multirow{2}{*}{\textbf{XLM-R}}             & MSE                   &                                  &                                  &                                                      &                                                     &                                         \\ 
% % \cmidrule{2-7}
% %                                             & Binary Classification &                                  &                                  &                                                      &                                                     &                                         \\ 
% % \midrule
% % \multirow{2}{*}{\textbf{IndicBERT}}         & MSE                   &                                  &                                  &                                                      &                                                     &                                         \\ 
% % \cmidrule{2-7}
% %                                             & Binary Classifiction  &                                  &                                  &                                                      &                                                     &                                         \\
% % \hline\hline
% % \end{tabular}
% % }
% % \end{table}

==> tables/04-results-join-training.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table*}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccc} 
\hline\hline
\multicolumn{1}{c}{}                                                           &                             &          & \multicolumn{8}{c}{Joint Training}                                                                                                                             \\ 
\cmidrule{4-11}
\multicolumn{1}{c}{}                                                           &                             &          & \multicolumn{4}{c}{OSN}                                           & \multicolumn{4}{c}{GCM}                                                                    \\ 
\cmidrule{4-11}
\multicolumn{1}{c}{}                                                           &                             &          & \multicolumn{2}{c}{Avg Rating} & \multicolumn{2}{c}{Sum Abs Diff} & \multicolumn{2}{c}{Avg Rating}              & \multicolumn{2}{c}{Sum Abs Diff}             \\ 
\cmidrule{4-11}
\multicolumn{1}{c}{}                                                           &                             &          & RMSE & MAE                     & RMSE & MAE                       & RMSE                 & MAE                  & RMSE                 & MAE                   \\ 
\hline\hline
Human Annotations Baseline                                                     &                             &          & \multicolumn{2}{c}{}           & \multicolumn{2}{c}{}             &                      &                      &                      &                       \\ 
\hline\hline
\begin{tabular}[c]{@{}l@{}}Feed-Forward Network \\- Code-mix Metrics\end{tabular} &                             &          & \multicolumn{2}{c}{}           & \multicolumn{2}{c}{}             &                      &                      &                      &                       \\
~~~ + MLLM Perplexity scores                                                   &                             &          & \multicolumn{2}{c}{}           & \multicolumn{2}{c}{}             &                      &                      &                      &                       \\ 
\hline\hline
\multirow{4}{*}{XLM-Roberta}                                                   & roman                       & Frozen   & 2.71 & 2.52                    & 2.72 & 2.14                      & 1.77 \textbar{} 1.33 & 1.51 \textbar{} 1.11 & 2.08 \textbar{} 2.17 & 1.59 \textbar{} 1.67  \\
                                                                               & \multicolumn{1}{l}{}        & Unfrozen & 0.95 & 0.8                     & 1.92 & 1.49                      & 0.89 \textbar{} 0.90 & 0.74 \textbar{} 0.74 & 1.88 \textbar{} 1.87 & 1.56 \textbar{} 1.52  \\
                                                                               & \multirow{2}{*}{normalised} & Frozen   & 2.3  & 2.08                    & 2.24 & 1.73                      & 1.51                 & 1.27                 & 2.07                 & 1.58                  \\
                                                                               &                             & Unfrozen & 0.91 & 0.85                    & 1.93 & 1.496                     & 0.83                 & 0.68                 & 1.87                 & 1.54                  \\ 
\midrule
\multirow{4}{*}{IndicBERT}                                                     & \multirow{2}{*}{roman}      & Frozen   & 3.4  & 3.26                    & 2.89 & 2.27                      & 2.75 \textbar{} 2.65 & 2.6 \textbar{} 2.48  & 2.74 \textbar{} 2.77 & 2.29 \textbar{} 2.31  \\
                                                                               &                             & Unfrozen & 1.02 & 0.87                    & 1.95 & 1.61                      & 0.9 \textbar{} 0.91  & 0.76 \textbar{} 0.77 & 1.84 \textbar{} 1.85 & 1.56 \textbar{} 1.57  \\
                                                                               & \multirow{2}{*}{normalised} & Frozen   & 3.4  & 3.26                    & 2.89 & 2.27                      & 2.63                 & 2.47                 & 2.67                 & 2.21                  \\
                                                                               &                             & Unfrozen & 1.01 & 0.86                    & 1.96 & 1.595                     & 0.9                  & 0.76                 & 1.87                 & 1.56                  \\ 
\midrule
\multirow{4}{*}{BERNICE}                                                       & \multirow{2}{*}{roman}      & Frozen   & 1.13 & 0.93                    & 1.99 & 1.62                      & 1.03 \textbar{} 1.03 & 0.84 \textbar{} 0.84 & 1.88 \textbar{} 1.89 & 1.6 \textbar{} 1.6    \\
                                                                               &                             & Unfrozen & 0.94 & 0.77                    & 1.91 & 1.54                      & 0.87 \textbar{} 0.87 & 0.7 \textbar{} 0.70  & 1.89 \textbar{} 1.89 & 1.5 \textbar{} 1.6    \\
                                                                               & \multirow{2}{*}{normalised} & Frozen   & 1.07 & 0.88                    & 1.94 & 1.5                       & 0.97                 & 0.8                  & 1.9                  & 1.6                   \\
                                                                               &                             & Unfrozen & 0.93 & 0.78                    & 1.92 & 1.53                      & 0.86                 & 0.69                 & 1.83                 & 1.53                  \\
\hline\hline
\end{tabular}
}
\caption{Results - Joint Training}
\label{tab:results_joint_training}
\end{table*}

==> tables/05-IAA.tex <==

\begin{table}[b]
% \vspace{0.5cm}
\centering
\resizebox{0.65\linewidth}{!}{%
\begin{tblr}{
  cells = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  hline{1,8} = {-}{0.08em},
  hline{2} = {2-5}{0.03em},
  hline{3} = {-}{0.05em},
}
{Disagreeement} & GCM   &                           & OSN   &                           \\
                                 & ICC1k & {\% of samples \\covered} & ICC1k & {\% of samples \\covered} \\
0                                & 1     & 16\%                      & 1     & 23\%                      \\
0-2                              & 0.92  & 58\%                      & 0.93  & 65\%                      \\
0-4                              & 0.79  & 87\%                      & 0.85  & 87\%                      \\
0-6                              & 0.68  & 98\%                      & 0.78  & 97\%                      \\
0-8                              & 0.66  & 100\%                     & 0.75  & 100\%                     
\end{tblr}
}
\caption{Inter-Annotator Agreement (ICC1k) for GCM and OSN data. Disagreement is calculated as sum of pair-wise absolute differences and quantifies the degree of disagreement between the three annotators. Samples where the Sum of Absolute Pair-wise Differences is $\leq4$ have good agreement (ICC1k between 0.7 and 0.9).}
\label{tab:IAA}
\end{table}




% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{llrrrrr} 
% \hline\hline
%                      &                       & \multicolumn{5}{l}{Sum of Pair Wise Difference}                                                                                        \\ 
% \cmidrule{3-7}
%                      &                       & \multicolumn{1}{l}{0}    & \multicolumn{1}{l}{0-2}  & \multicolumn{1}{l}{0-4}  & \multicolumn{1}{l}{0-6}  & \multicolumn{1}{l}{0-8}    \\ 
% \midrule
% \multirow{3}{*}{GCM} & \% of Samples Covered & \multicolumn{1}{l}{16\%} & \multicolumn{1}{l}{58\%} & \multicolumn{1}{l}{87\%} & \multicolumn{1}{l}{98\%} & \multicolumn{1}{l}{100\%}  \\
%                      & Krippendorff's Alpha  & 1                        & 0.8                      & 0.55                     & 0.39                     & 0.39                       \\
%                      & ICC2k                   & 1                        & 0.92                     & 0.79                     & 0.68                     & 0.66                       \\ 
% \midrule
% \multirow{3}{*}{OSN} & Num of Samples        & 23\%                     & 65\%                     & 87\%                     & 97\%                     & 100\%                      \\
%                      & Krippendorff's Alpha  & 1                        & 0.75                     & 0.65                     & 0.52                     & 0.52                       \\
%                      & ICC2k                   & 1                        & 0.93                     & 0.85                     & 0.78                     & 0.75                       \\
% \hline\hline
% \end{tabular}
% }
% \caption{Inter-Annotator Agreement}
% \label{tab:IAA}
% \end{table}

==> tables/error_analysis_correlation.tex <==
\begin{table}
\centering
\caption{Correlation between prediction error and code-mix metrics indicate that there aren't any clear correlation between the prediction error and the code-mix metrics of the samples}
\begin{tabular}{lrr} 
\hline\hline
                       & \multicolumn{1}{l}{GCM} & \multicolumn{1}{l}{OSN}  \\ 
\hline\hline
Length                 & -0.039                  & 0                        \\
CMI                    & -0.0035                 & 0.012                    \\
SPAvg                  & 0.054                   & 0.038                    \\
Burstiness             & -0.019                  & 0                        \\
SyMCoM Sentence Scores & -0.033                  & 0.049                    \\
Surprisal              & 0.08                    & 0.2                      \\
\hline\hline
\end{tabular}
\end{table}

==> tables/error_analysis_symcom_anova.tex <==
% \usepackage{colortbl}


\begin{table}
\centering
\caption{One way ANOVA analysis between PoS tag wise SyMCoM scores. We convert SyMCoM values into categories to encode if a particular PoS tag is mixed or monolingual or not present in the text.}
\begin{tabular}{lllll} 
\hline\hline
      & \multicolumn{2}{c}{\textbf{GCM}}                                                      & \multicolumn{2}{c}{\textbf{OSN}}                                                       \\ 
\hline\hline
      & F-statistic                               & p-value                                   & F-statistic                               & p-value                                    \\
ADJ   & {\cellcolor[rgb]{0.984,0.714,0.725}}1.794 & {\cellcolor[rgb]{0.973,0.506,0.518}}0.167 & {\cellcolor[rgb]{0.984,0.796,0.808}}1.325 & {\cellcolor[rgb]{0.976,0.561,0.569}}0.267  \\
ADP   & {\cellcolor[rgb]{0.976,0.502,0.51}}3.055* & {\cellcolor[rgb]{0.973,0.424,0.431}}0.048 & {\cellcolor[rgb]{0.984,0.82,0.831}}1.161  & {\cellcolor[rgb]{0.976,0.592,0.6}}0.314    \\
ADV   & {\cellcolor[rgb]{0.988,0.969,0.98}}0.273  & {\cellcolor[rgb]{0.984,0.925,0.937}}0.761 & {\cellcolor[rgb]{0.988,0.847,0.859}}0.989 & {\cellcolor[rgb]{0.976,0.627,0.635}}0.373  \\
AUX   & {\cellcolor[rgb]{0.988,0.969,0.98}}0.270  & {\cellcolor[rgb]{0.984,0.925,0.937}}0.764 & {\cellcolor[rgb]{0.988,0.922,0.933}}0.497 & {\cellcolor[rgb]{0.98,0.773,0.784}}0.609   \\
CCONJ & {\cellcolor[rgb]{0.988,0.988,1}}0.147     & {\cellcolor[rgb]{0.984,0.882,0.894}}0.702 & {\cellcolor[rgb]{0.984,0.835,0.847}}1.057 & {\cellcolor[rgb]{0.976,0.612,0.62}}0.348   \\
DET   & {\cellcolor[rgb]{0.988,0.91,0.922}}0.632  & {\cellcolor[rgb]{0.98,0.765,0.773}}0.531  & {\cellcolor[rgb]{0.98,0.627,0.635}}2.433  & {\cellcolor[rgb]{0.973,0.451,0.459}}0.089  \\
INTJ  & {\cellcolor[rgb]{0.98,0.631,0.643}}2.283  & {\cellcolor[rgb]{0.973,0.482,0.49}}0.131  & {\cellcolor[rgb]{0.988,0.988,1}}0.050     & {\cellcolor[rgb]{0.988,0.988,1}}0.951      \\
NOUN  & {\cellcolor[rgb]{0.984,0.82,0.831}}1.160  & {\cellcolor[rgb]{0.976,0.612,0.62}}0.314  & {\cellcolor[rgb]{0.973,0.412,0.42}}3.832* & {\cellcolor[rgb]{0.973,0.412,0.42}}0.022   \\
NUM   & {\cellcolor[rgb]{0.984,0.804,0.816}}1.256 & {\cellcolor[rgb]{0.976,0.592,0.6}}0.285   & {\cellcolor[rgb]{0.984,0.816,0.827}}1.199 & {\cellcolor[rgb]{0.976,0.565,0.576}}0.274  \\
PART  & {\cellcolor[rgb]{0.988,0.969,0.98}}0.269  & {\cellcolor[rgb]{0.984,0.925,0.937}}0.765 & {\cellcolor[rgb]{0.988,0.871,0.882}}0.833 & {\cellcolor[rgb]{0.976,0.667,0.675}}0.435  \\
PRON  & {\cellcolor[rgb]{0.988,0.945,0.957}}0.423 & {\cellcolor[rgb]{0.984,0.851,0.863}}0.655 & {\cellcolor[rgb]{0.98,0.616,0.624}}2.506  & {\cellcolor[rgb]{0.973,0.447,0.455}}0.082  \\
PPRON & {\cellcolor[rgb]{0.973,0.412,0.42}}3.584* & {\cellcolor[rgb]{0.973,0.412,0.42}}0.028  & {\cellcolor[rgb]{0.988,0.875,0.886}}0.809 & {\cellcolor[rgb]{0.976,0.675,0.682}}0.446  \\
SCONJ & {\cellcolor[rgb]{0.988,0.988,1}}0.164     & {\cellcolor[rgb]{0.988,0.988,1}}0.849     & {\cellcolor[rgb]{0.98,0.643,0.655}}2.315  & {\cellcolor[rgb]{0.973,0.459,0.467}}0.100  \\
VERB  & {\cellcolor[rgb]{0.98,0.604,0.612}}2.449* & {\cellcolor[rgb]{0.973,0.451,0.459}}0.087 & {\cellcolor[rgb]{0.988,0.953,0.965}}0.287 & {\cellcolor[rgb]{0.984,0.863,0.875}}0.751  \\
\hline\hline
\end{tabular}
\end{table}
